MonoGaussianAvatar: Monocular Gaussian Point-based Head Avatar

The ability to animate photo-realistic head avatars reconstructed from monocular portrait video sequences represents a crucial step in bridging the gap between the virtual and real worlds. Recent advancements in head avatar techniques, including explicit 3D morphable meshes (3DMM), point clouds, and neural implicit representation have been exploited for this ongoing research. However, 3DMM-based methods are constrained by their fixed topologies, point-based approaches suffer from a heavy training burden due to the extensive quantity of points involved, and the last ones suffer from limitations in deformation flexibility and rendering efficiency. In response to these challenges, we propose MonoGaussianAvatar (Monocular Gaussian Point-based Head Avatar), a novel approach that harnesses 3D Gaussian point representation coupled with a Gaussian deformation field to learn explicit head avatars from monocular portrait videos. We define our head avatars with Gaussian points characterized by adaptable shapes, enabling flexible topology. These points exhibit movement with a Gaussian deformation field in alignment with the target pose and expression of a person, facilitating efficient deformation. Additionally, the Gaussian points have controllable shape, size, color, and opacity combined with Gaussian splatting, allowing for efficient training and rendering. Experiments demonstrate the superior performance of our method, which achieves state-of-the-art results among previous methods.

==> sections/11111.tex <==
\section{Introduction}
\label{sec:introduction}
%
% In the realm of augmented reality (AR) and virtual reality (VR) telepresence applications, the automatic construction of personalized 3D head avatars from monocular portrait videos represents a crucial advancement that bridges the gap between the physical and digital worlds.
The urgent demand for automated construction of personalized 3D head avatars from monocular portraits is underscored by the evolving landscape of AR and VR wearables, such as Apple Vision, PICO, etc.
%
These avatars must meet the demanding criteria of photorealistic facial geometry, intricate facial appearance, and precise representation of dynamic expressions to fulfill the expectations of users.
%
% Such an avatar requires photo-realistic facial geometry, detailed facial appearance, and accurate deforming expression to satisfy the demands of users.
%

%
% Recently, there have been three approaches commonly employed for constructing 3D head avatars from portrait videos: 3D Morphable Model (3DMM){\cite{blanz2023morphable, li2017learning, paysan20093d}}, Neural implicit representation {\cite{mescheder2019occupancy, park2019deepsdf, mildenhall2021nerf}}, and others explicit representation {\cite{zheng2023pointavatar}}.
Recent efforts have pursued three primary presentations for the creation of 3D head avatars from portrait videos: the 3D Morphable Model (3DMM), Neural implicit representation, and other explicit representations, IMavatar and PointAvatar.
% 3DMMs can efficiently represent facial geometry and are capable of generalizing to unseen deformations. However, the template mesh is a pre-defined fixed topography and is constrained to surface-like geometries, which struggle to model eyeglasses, hair, and other wearings.
3DMMs{\cite{blanz2023morphable, li2017learning, paysan20093d}} excel in efficiently representing rough facial geometry and have the capacity to generalize to novel deformations. However, they are limited by their predefined fixed topologies and are constrained to surface-like geometries, making them less suitable for modeling features such as eyeglasses, hair, and other accessories.
%这段需要修改
Neural implicit representations{\cite{mescheder2019occupancy, park2019deepsdf, mildenhall2021nerf}} can be categorized into NeRF-based and SDF-based methods. The former strengthens in capturing intricate details such as hair strands and eyeglasses, while the latter demonstrates strength in reconstructing geometry. 
%
% However, they are less efficient in terms of training and rendering since generating a single pixel involves querying numerous points along the camera ray.
Nonetheless, their efficiency in training and rendering is compromised, as generating a single pixel necessitates querying numerous points along the camera ray.
%
% Furthermore, deforming implicit representations in a generalizable manner is a non-trivial task, often entailing inefficient root-finding loops, which negatively impact both training and testing times.
%
% Other explicit representations, such as PointAvatar{\cite{zheng2023pointavatar}}, strengthen in both modeling complex hair geometry and efficiency of rendering.
% We consider PointAvatar{\cite{zheng2023pointavatar}} as an example for other explicit representations.

%
For other explicit representations, PointAvatar{\cite{zheng2023pointavatar}} stands out as an exemplary model showcasing superior performance compared to other methods.
%
Compared to implicit representations, points can be rendered efficiently with a standard differentiable rasterizer and deformed efficiently using learned blendshapes and skinning weight from pre-trained 3DMM (FLAME) with a given expression and pose.
%
Compared to meshes, they are considerably more flexible and versatile, which confirms the topology of accessories such as glasses and complex volumetric structures such as hair.
%
However, PointAvatar fixes its rendering radius uniformly which increases the number of required training points, imposing a heavier training burden.
%voids
It also results in a number of holes when the face undergoes substantial movement.
%
Moreover, since the deformation of points is learned through Linear Blend Skinning (LBS), certain rigid parts such as teeth may undergo similar deformation as the lips, leading to inaccuracies.
%

%
In this paper, we introduce Monocular Gaussian Point-based Avatar (MonoGaussianAvatar), which utilizes 3D Gaussian points to represent the facial appearance and geometry while integrating a continuous Gaussian parameter deformation field along with a point deformation field for animation.
%
Our 3D Gaussian points are characterized by 5 Gaussian parameters: mean position, albedo color, opacity, rotation, and scale. Compared to 3D Gaussian splitting (3D-GS{\cite{kerbl20233d}}), we directly utilize a 3-channel RGB albedo color to replace the color of the radiance field represented via spherical harmonics (SH).
%
We perform a mapping of the mean position to the other Gaussian parameters in canonical space to establish the canonical 3D Gaussian points.
%
Specifically, albedo color is a pose-agnostic parameter that is directly calculated from this mapping in canonical space and fixed in deformed space.
%
For animation, the learned Gaussian parameter deformation field maps the motion of mean position to the offsets of other parameters between canonical and deformed space.
%
Compared to PointAvatar, these Gaussian parameters facilitate more efficient rendering thanks to 3D-GS, which also provides points with a more flexible shape and size to compensate for the holes of conventional point rendering. 
%
Simultaneously, because of its anisotropy, the number of points for a similar quality rendering to PointAvatar is reduced, which means that more Gaussian points can be utilized to improve the details of rendering.
% Thanks to 3D Gaussian splitting, these parameters facilitate more efficient rendering in comparison to conventional point-based differentiable rasterizers and neural rendering.
%
% In terms of point deformation, We perform a mapping of the mean positions of 3D Gaussian points from canonical space to deformed space, drawing inspiration from PointAvatar.
% %
% This mapping is accomplished by employing learned blendshapes and skinning weight derived from a pre-trained 3DMM (FLAME) with a given expression and pose.
% %
% Compared to the mesh-based method, 3D Gaussian points representation offers more degree of freedom, allowing us to circumvent the constraints associated with fixed topologies limited to the mesh surface.
%
% Moreover, the rotation and scale of 3D Gaussian points can compensate for holes while simultaneously reducing the number of points required for rendering, in contrast to conventional point-based rendering. 
%

%
% One strength of our method is that we first introduce 3D Gaussian representation in head avatar work, along with a Gaussian parameters deformation field for animation.
% One strength of our method is that we introduce a mapping of the mean position to the other Gaussian parameters in canonical space to form a 3D Gaussian points representation, along with a Gaussian parameters deformation field for animation.
% %
% This innovation allows for a seamless transition from original static 3D Gaussians to dynamic representations.
One strength of our method is that we achieve a seamless transition from original static 3D Gaussians to dynamic representations.
%
Compared to 3D-GS which relies on iteration optimization for parameter updates and implements point insertion and deletion based on adaptive density to reconstruct scenes, we propose a Gaussian prediction network to predict Gaussian parameters in canonical space and a Gaussian deformation field for animation.
%
Due to the discrete nature of Gaussian points, simply utilizing RGB loss to constrain the deformation of point position and head geometry presents a formidable challenge.
%
Consequently, we introduce an innovative strategy involving point insertion and deletion to enhance training stability and boost convergence efficiency.
%
The application of these techniques collectively contributes to the high-quality estimation of Gaussian parameters, resulting in significant improvements in both the geometry and appearance of the 3D head Avatar.
%

%
We compare our method with the state-of-the-art (SOTA) method using structure similarity, image similarity, and Peak Signal-to-Noise Ratio.
%
% We quantitatively demonstrate that our method generates better unseen expressions and poses with more accurate appearance and geometry than those SOTA techniques.
Our quantitative assessments conclusively reveal that our method excels in generating previously unseen expressions and poses, delivering superior results in terms of both appearance and geometry when juxtaposed with the SOTA methods.
%

\medskip
\noindent
 
The contributions of this work are as follows:

\begin{itemize}
    \item We first present a Gaussian point-based explicit head avatar model which is combined with facial expressions and poses that can reconstruct detailed geometry and appearance from monocular videos.
    
    \item We introduce a strategy of Gaussian points insertion and deletion, which significantly enhances the stability of training and improves convergence efficiency.
    
    \item We present an improvement of the Gaussian points setting, the optimization of Gaussian parameters, and the Gaussian deformation field regarding 3D Gaussian splitting, which shows state-of-the-art photo realism while achieving real-time rendering.

    %\item Our method recovers detailed wrinkles of head avatars just on monocular videos, which also achieves real-time rendering.
    % \item The framework achieves real-time rendering on human avatars, up to 30 FPS at a resolution of $1024 \times 1024$, while containing comparable performance with state-of-the-art methods.
\end{itemize}
% efficient 4D Gaussian representation by modeling the Gaussian parameters prediction field and Gaussian deformation field, which can be combined with facial expressions and poses to reconstruct 3D head avatars from monocular videos.

 % We introduce a set of point insertion and deletion strategies and, with the assistance of Gaussian rendering, enable the reconstruction of a dense point cloud avatar of a human head from a randomly initialized sparse point cloud.
